Advanced atom-level representations for protein flexibility prediction utilizing graph neural networks

Protein dynamics play a crucial role in many biological processes and drug interactions. However, measuring, and simulating protein dynamics is challenging and time-consuming. While machine learning holds promise in deciphering the determinants of protein dynamics from structural information, most existing methods for protein representation learning operate at the residue level, ignoring the finer details of atomic interactions. In this work, we propose for the first time to use graph neural networks (GNNs) to learn protein representations at the atomic level and predict B-factors from protein 3D structures. The B-factor reflects the atomic displacement of atoms in proteins, and can serve as a surrogate for protein flexibility. We compared different GNN architectures to assess their performance. The Meta-GNN model achieves a correlation coefficient of 0.71 on a large and diverse test set of over 4k proteins (17M atoms) from the Protein Data Bank (PDB), outperforming previous methods by a large margin. Our work demonstrates the potential of representations learned by GNNs for protein flexibility prediction and other related tasks.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> tables/egnn_results.tex <==
\begin{tabular}{llllllll}
\toprule
{} &           cc &           mae &             mse &         mape &         rrse &            r2 &           kl \\
dataset &              &               &                 &              &              &               &              \\
\midrule
test    &  0.64±0.0234 &   13.52±0.782 &   388.03±52.678 &  0.39±0.0074 &  1.17±0.0536 &  -0.76±0.0732 &  0.05±0.0018 \\
train   &  0.65±0.0104 &   12.16±0.206 &  300.38±25.5548 &   0.5±0.0334 &   1.22±0.015 &  -0.76±0.0454 &  0.05±0.0006 \\
valid   &   0.66±0.009 &  12.74±0.1568 &  338.98±25.1532 &  0.57±0.0424 &  1.28±0.0274 &  -1.15±0.0748 &  0.05±0.0008 \\
\bottomrule
\end{tabular}


==> test_codes.tex <==
5lct,4l7f,5s75,7ajs,5l8k,5ntj,4nif,4asz,4uwb,5oot,3gbz,2r3q,6vhg,4rx9,6gl9,2itv,5orv,2o63,5e91,3fsf,1qmz,5r97,5hu3,5s86,1q3d,6x5g,2e9u,7c3n,6zcy,6ypg,2r0u,7c2v,5n3o,5nhp,2jko,6n8g,4ji9,1r3c,2ym3,3qzf,6yna,5awm,6vnb,4ie9,7a2h,7b3w,5m0l,4x2f,5ots,2jam,2vu3,1xh9,7fd0,5n4r,3q9z,4bib,5a4q,2xf0,5t1h,6n7d,3e8c,7nqw,3u4u,6mt0,3sv0,6eii,6f3i,6z56,5r9x,4kio,4m15,6pdn,4u41,6drw,4fsm,3sa0,5p9f,1u5q,3da6,3u6i,6rcm,4eop,5s7z,6v66,3gu5,4aa4,3kn6,6p5s,2a0c,4jjr,4fyo,4i0r,3zrk,6spm,7f3g,2w9z,4hgs,3q52,4d4v,6qtj,4f9w,6hbn,5iex,4c33,3r04,4hyu,3blh,6l24,3uvq,4e5w,4pqn,6hoq,5izf,7kac,1ckp,5h0e,1tqi,1wbw,4qmm,4rvm,6fin,3w8l,4zy5,6qav,6hes,5i9z,4jdi,7kja,2yac,1q62,1h27,3oxi,3l8v,6rsh,6eiq,6vg3,6yg0,6e2n,4fij,5s8a,4fsu,4wb7,1yoj,6ot6,3rm6,6r8j,3lau,4fnw,1m2q,5s7b,3ork,1yhw,5k7g,2qd9,4d0w,6e0r,3a7h,2ojf,6q4j,4fkv,4f0i,6gql,3owj,1wak,4xh6,6spu,6iuo,5ax9,3tei,6fnk,4x21,2x0g,6g9j,1cdk,6fyk,3x2u,7kie,4f4p,3bqr,6yk7,1opk,3r71,6emh,7fcz,2b7a,7jxy,1o9u,6h3k,3com,2oib,2vwx,1wbo,6hzu,4qmu,1v0o,6erv,6isj,3agm,5r8x,4lg4,3unj,3l9n,6bg2,6xx7,7t4m,5y5t,2pzi,5opr,3qyz,6v6a,3be9,3gub,2rei,5x1t,6xdb,3cd8,5vcw,5ous,2r3i,3dkc,4whz,4a7c,6q38,5orn,5cas,2dyl,7o7k,6lxy,6z5a,6sm8,3rhx,7a6i,2uw0,2exm,5uzk,4yne,7oak,5tel,5nhh,5mai,6tfz,7avq,5jn2,2qol,2h8h,6z4y,4m0z,5wil,5jk3,5n1k,2xk7,2b52,1j1b,4qp8,2ok1,2pvn,2izu,7mon,5ra4,6y7z,4twc,5cxh,7r60,2jdt,6vnf,4bkz,7ju5,5b7v,3f3z,5osj,4lgg,1svg,6ykd,5n3k,2ym7,5lmk,4o0x,3fmd,2jkk,7d57,5auu,6ep9,5n4v,7ako,2of2,3eyg,1b39,3fxx,6tsz,6eg9,2qhm,1q8z,7n5r,2pvr,2fsl,5oop,6q49,3roy,5ttu,3ns9,7axv,5lcp,3qcy,6npe,6a1f,4ytf,5lvl,5clp,5s82,6uya,5g15,5orr,3pwd,4acc,5r93,2hxl,5mmr,4tnd,6ebw,4d1s,3t3u,3r00,6yl6,5ihc,6ggh,6hou,2iw9,4d4r,6i5k,2xkd,6pxp,6jut,4c37,3py0,2c1a,3mtl,3hv6,6ehu,4ot6,4feq,6hwv,6hew,3ha6,2xix,3vbv,3pa3,3iw7,1tqm,4pmp,3u9n,4iak,6tg1,4l00,4o91,3e63,4an3,3a8w,4dli,7suf,5we8,3obj,3cqw,4ct2,5vd9,7nr8,1apm,3fi2,4eev,6eas,6l14,4d2w,6pdj,1yxv,1v1k,6eim,6z52,6gqp,6dbn,4fkj,3bhu,6s9w,6pcw,6j5l,6s1i,7aj8,4ftt,1wvw,1h07,2b9f,4aa0,4xw4,6fyo,3rk7,3mvh,4hcv,5dey,2w5a,3w2r,4hyi,4d9u,3g51,6sfi,3nww,6n77,6mm7,7ay9,7kia,4jnw,1ydt,4aw0,4qps,6jgm,6inl,6vs3,2bfx,1nvs,3ovv,3cek,6g9n,6kyr,3mfu,6o95,4mq1,4qmq,3txo,5e8z,3sw4,6hmq,3o8u,5f9e,3gi3,4mf1,5h8g,6y82,4bf2,6fdm,6b16,4yo6,6ny4,3coi,4fsq,5eob,5ita,3oom,4at4,3qd3,3mpm,3tnw,2yiy,3ccn,4fvp,6w06,3pe2,2eu9,5r9d,6yg4,4rwi,4m97,2xmy,6rfp,3pj1,4jbp,4fkr,4oh4,1oit,3oro,5s7f,2x4z,1yhs,1zar,3kf4,4dym,5aep,6ccy,5bvn,2qoh,5osr,2jfl,1day,5nhl,5t6i,5n3s,2r0i,3piz,5cen,7rj6,3she,5t1t,5n4n,5ra0,2c47,5ih4,7bjh,2vx0,6urc,6sk9,3mi9,1stc,4wsy,5n1o,7ccw,2xk3,5oto,4zlz,2pvj,2vo0,2fst,3f5g,3p1a,1qpd,2erk,5nkh,3dqx,3dkg,2w17,2r3m,4o6e,5eh0,5o1v,5opv,2ivv,7m0l,5ia2,6eq9,6y6f,5m4i,5buj,5mov,5anj,2wu6,7q90,7b7r,2uw4,6lub,2q0n,5csv,5umo,7bar,5orj,3vf8,6tpf,7cml,5dt3,6z5e,3dlz,6z4d,2qoq,5bvw,5t3q,6yfz,5ywm,5n3j,3wf8,2duv,7cil,3fme,6xoe,4o0y,2ym6,5a4t,5aut,6n7a,1b38,2w06,5tos,7ops,6bhc,5oni,2j2i,6nzf,6q48,2fsm,7ra5,3pxf,3rgf,2xj2,3qtx,7b8h,5lcq,7axw,5uoj,7ajv,2qlu,5k75,3qcx,3dfa,7e73,5s83,5lvm,4zog,6a1g,5owr,5wev,7cht,7rn6,5u6i,5ors,6cpy,4xoy,5hg7,5r92,6l1z,4aqc,1o6k,1zzl,6l21,6fyv,6snn,2iw8,6hot,6guh,6juu,4gfm,6z36,2x8d,2xke,6egw,6itj,4nm5,4d4s,4uv0,4c36,4eym,6dki,3py1,4ekl,3hv7,6qas,6hev,5eyc,3ocs,2xiy,6y05,4hvs,2uvz,6q7s,3iw6,3u8w,3vbw,7dua,6tg0,6t41,4erw,3e62,4l01,4pwn,4u44,4c02,1ke5,7sug,3mpt,3oxt,6rij,3fi3,3lct,5e1e,7nr9,5vd8,6gdm,6eil,6z53,3dv3,3nnu,4daw,4d2v,2vta,6hkm,6gqq,6rfi,6s1h,4dtk,3bht,1zlt,4d5k,3hp2,4ftu,6wa2,6ne7,3fc1,6rch,3bwj,6cz4,6i1s,6sov,4xw5,4as0,4d9t,4hyh,3war,3w2s,4rfm,2cgx,6mm6,2bfy,3gc0,4aw1,1nvr,4o22,5kgg,2nry,4qmp,3w8q,3mft,6ers,3o8t,6bu6,3lxk,2c6e,5hcy,1zoh,6q7k,4pdo,4jik,3lok,4xp0,4at5,3tti,4uj2,3v5w,3l8s,6w07,4fvq,2uze,2yix,4wg3,6yg5,5r9e,4fks,4jbq,3s00,5o49,6p8q,3hx4,4qqj,1oiu,5gza,5s7g,4eom,4ftm,1py5,3k54,5mo8,6jkk,6fxv,5bvo,2qoi,4apc,7lvi,5j87,5fp5,3a99,5n3r,6y0b,4agc,7rj7,5lwm,2v62,2ijm,5ceo,5n4o,5ra1,4usf,2vx1,5ih5,4zse,7ccv,5n1n,5wfj,3qgy,2pvk,3e5a,5uyj,5ooi,1qpe,2f2u,2r3l,3dkf,6vre,1p5e,5nki,5ugl,5ia3,7m0m,3ggf,4brx,5mow,2hzi,2wu7,5ank,5x1q,2oh0,2uw5,3f7z,4cqe,5k00,5l2t,3vf9,6x8e,5ork,2rgp,2gph,6z5d,4bbe,5l8j,5v5n,2pzp,6thx,5cyi,5lcu,2qlq,5t8o,3pjc,4uwc,6t6f,4rx8,3d0e,2r3p,3we8,4uja,5orw,5e90,6aub,5r96,2g1t,4wua,3g6g,3fly,4ytc,6a1c,5s87,6zcx,2gtm,5n3n,2zv2,3ot8,7dt2,2ptk,6p69,6cqe,4xne,4axa,3qzg,5jq5,7b3v,4x2g,1e1x,3qud,5n9l,1xh8,5otr,4f99,5hd7,3jya,3vnt,6l11,4kin,6pdo,4m14,4d2r,5r9y,2xez,1yxs,6z57,5p9g,4ian,3v8t,4u40,3lfq,1lpu,5h9b,4ftq,4eoq,3umw,6nw2,6gtt,3pg3,3u6h,3iq7,4e4n,2ycf,4aa5,3aln,3gu4,1zao,6n33,5cf8,6dbk,4i0s,4fyn,4fko,3q53,4dfn,6spl,4qyh,5drd,5khx,2qr8,5to8,3b2w,6cd6,5iey,5hvy,6fyr,3qx4,5dmz,6hop,3uvp,6yq1,1pw2,3byu,6j6m,7q8z,3uys,1wbv,3f61,6fio,3hv3,4qml,4wt6,6lk6,4rvl,4jdh,4f6u,4z84,6qaw,6gdq,1h26,6hdr,7que,2yab,5r9a,6zn0,4xg4,6e2o,6frp,4rwl,4tn6,1xkk,4pmm,4fst,4erk,6gin,1sm2,3rm7,5hbe,4wb6,6srh,6rct,4eoi,3lij,4fti,3i81,5s7c,4itj,3fy2,1m2p,4h1j,3a7i,1yhv,7qhg,3owk,4ebv,4fkw,6q4k,1m7q,2ojg,3bhh,1oiq,4aw5,4dgn,6itv,6fnj,3dj5,3d94,4nw6,4pni,6qfr,6xe4,3ig7,6g9k,4xv1,3r83,3mvm,3bym,1cki,6flv,5n39,1opj,4kwp,1wbn,2vwy,2oic,1tqp,5r8y,6erw,3agl,1ykr,4rvt,3nun,4bc6,4qmt,5n68,2w7x,5hnb,5nw8,5os8,2vrx,3unk,6xx6,3o8p,4p2k,3cs9,3poz,5ops,2ivs,5jh6,2cn5,5y5u,3r9d,5ano,3pxz,6xvb,4d58,5w4w,2r3h,5oro,4y8d,4h39,4w4y,6cpe,2hxq,2oh4,6v9c,5tvt,7oaj,6zjf,2gnj,5twl,2xa4,3g2f,2j0i,6ytg,4a9y,4otd,3p7a,5m0u,4qp9,4mvf,2b53,2xk6,2r2p,2izt,7n5o,5z0s,6hp9,7a5l,7dv6,2g2h,5ke0,5ra5,4zsa,3vw8,7r61,5vgo,2j7t,5o8u,7bjm,7b9l,3eqd,6rcg,5s7p,5c03,2w4o,5d7v,5tq5,2b9h,5oo1,2vtn,5y86,6rff,7f3m,5nk1,5wo4,3qf9,7kjs,5vd7,6c19,4g3f,1yxx,5r9r,7aw4,5ya5,5p9l,5mz3,7suh,4xx9,2qq7,7jys,2qc6,4dea,6e6e,6fle,7r9n,2chl,5s9k,6gzd,3uqf,3vbx,6sdc,5am7,6hey,3lpb,6gmd,5fxs,7b32,2z2w,4j7b,4pte,5ot6,6i8z,6fcf,4rfz,3du8,5i3r,5jsm,5oq7,1t45,4zji,7m2f,1rdq,3bu6,5hu9,5hg8,4acm,6bkh,4yth,4y5h,4obo,6wtn,1z57,6y9s,6zcs,4tyj,1irk,5mrb,7apf,1h0v,3fko,4ft5,7ajy,3w33,6ib2,3ad4,5ew8,5o4a,5oua,4ylk,4gg5,4xhk,5mja,5gz9,3qtw,3rtp,4awi,4dg2,6aam,3efw,6g97,3lw0,5oty,1q8t,5n4x,5xka,3qxp,3bv2,6c2r,4k11,4gk2,5cxz,5oyf,1q5k,3s4q,6w3k,7aka,5n3e,3wf7,4btj,3k3i,3fmj,3ot3,6di5,6g35,4dh1,3ral,2gqg,6vnh,3kmw,6qa3,5osd,6xjk,5yvb,3erk,3zo4,4lfi,6hd6,4fv1,4g31,4qd6,4mbi,6y4t,7du9,4yno,1jam,6ots,3ac1,3dak,5cyz,5ugc,7aja,3fqh,6v6k,3r1q,5and,3r9o,4gj2,6y6h,1s9j,1qpj,6nzq,6bss,6n3o,4c2v,4csv,3pxq,5nkf,4gt4,3gcp,4wih,6tlr,3s1h,4ek4,3nw6,3kul,5a4c,7ltz,3f9n,6x3p,4zsj,3qwk,6cnh,4fz6,6tfp,6bxi,6d22,6hh1,6bbv,2qof,5wax,4b8m,6fi3,3qrj,5uvf,1daw,6t8n,4s30,4yjv,4loo,7bk1,7ab0,5s7h,5mo7,5hes,1lez,4qtd,5jms,2pe2,6d1y,6g8x,4e6a,6rsb,2yiw,5c27,5r9j,3i79,5z33,5eol,6emb,5n32,6p3d,1zog,4hvd,6q7d,5hni,2bak,5k4i,5n63,4g2f,2qu6,3cjf,1gz8,5os3,5o23,5e8t,2wqn,4wa9,3p08,3ody,7k7q,5cu2,2vgo,5kmj,5hvj,5dew,3rk9,5ut5,2yjs,5fri,2cgw,6n79,3mtf,3nuy,6hmc,7b36,5ipj,4dee,3tub,2xir,7be6,1xjd,2y6m,7p3v,3amy,2xno,6guc,4i4e,7b94,6p1d,2qr7,2wkm,5ap1,5uy6,5iev,4f9y,2vtj,5idn,5n84,5nk5,2b4s,4qyg,5jrq,7aj2,5s7t,7dhh,4ow8,6dud,7khk,5uu1,5tc0,2wot,3nlb,2wgj,2w4k,5p9h,3zbx,6kzd,7aw0,6dmg,4c58,5vd3,2clq,4iva,6hvd,5av4,5r9v,2wev,6f3g,4grb,3mv5,1yi6,4xlv,7ake,6nvj,5m0b,5nxc,3enm,4ix5,1xh7,6brw,7n5x,6g93,3igo,4app,6vnl,5x2f,4dh5,3qzh,3rah,3hll,4bcn,6eh0,4f65,5ved,2c69,1gzk,4u0i,5xvg,1erk,3q6w,1ob3,2gfc,5n3a,5lma,4o0r,4ei4,4fr4,3fwq,6di1,3fmn,2vv9,3s2p,6gi6,4cki,2i0y,5s88,3hzt,3rwp,6vpj,4kd1,3zu7,4cfv,5orx,1mq4,4fl2,4cnh,4gh2,5r99,2r4b,3g6h,6pl1,4wun,3f5u,3ow3,3vs6,5oue,5zxb,6nzm,1jks,3qts,4mwi,3kkv,5bpy,3mh3,6vrv,4wrs,6thw,6g54,3zm4,7a1b,6so2,3qcs,1vr2,3qkm,6f14,5mod,4x7q,1pxi,6umw,6ylk,5vua,7aqb,2jld,4cmt,1h1r,5njz,4trl,4m7i,6y2u,4tzr,3hyh,2xk9,5n1e,5ote,6tlv,6nss,3efk,4czt,3sxr,3rin,2qob,5bvd,4j71,4yjr,6k74,4yxs,6tcu,6yqi,1ian,5nhf,5mag,5uab,3e7v,3uc4,3fln,6x5q,6xfp,4xbu,3bx5,5aac,4cfn,4fv5,1gij,4zxt,1zy4,6u5l,6uns,3geq,4n0s,4w4v,5z1d,5vcy,3i5n,6db3,6xdl,5nkb,1jkk,6s14,2r3g,4z3v,2og8,5v5y,7a1z,1hck,3qqj,5m4c,6v6o,6sg4,5r8v,6i2d,4gsb,7sqm,5n67,5os7,5v62,3zfy,6xx9,3ztx,7a21,5n36,6fvf,6z19,4p7e,1xbb,5dwr,5kmn,2wnt,5w80,3ama,4k1b,4kbc,6ti8,7ak2,5ut1,5vo1,4e5a,3jy9,2a4l,2xch,6egd,2bts,2w0j,7b43,5cu6,3vry,6r4c,6g9d,4f9a,5uq0,2vtr,5vc6,4f0g,6q4d,4hge,5s7l,5o13,2ycq,4fny,3a7f,4kke,5qil,5k7i,4iay,3lff,3oog,6fma,7jyo,2xzs,2yis,2uzn,3l8x,4uj9,7kxn,7nh5,5r9n,2bzh,2hy0,5m71,3p78,5uv4,2j51,5i9u,6hmb,2bdw,1ia8,3tuc,2x2l,5dpv,7l25,6mx8,3c4e,2z7s,5kwh,4d1x,7q7w,5zn4,4yz9,2ofv,4gfg,5ap0,4d4y,7a55,7at5,5ot3,5v80,4o38,4qyf,6s1b,5nk4,3kk8,6rcb,5s7u,2w4j,3tiy,3bea,2wou,5w91,7aw1,5p9i,5ftq,6z08,6hve,7nr3,2uzw,4s2z,4g3c,6z59,6eif,2bro,2g15,5r9w,7pqs,2np8,4azs,1pxp,6zwr,6csw,3r0t,4x7h,1om1,5lpb,2eva,3p5k,6nvk,6in0,5wnf,5m0c,3kxn,1p4o,1oz1,6omu,1e1v,6aah,6g92,2pvy,7n5y,1xh6,4ix4,6hx1,6tlo,4i94,3iop,1fvt,3qzi,4bco,3rai,6vnm,3pvw,6xbp,3fzo,1aq1,2c68,4f64,6ge0,4otr,7ore,4n4s,3krl,4nus,3dzq,3r7i,5usz,3e7o,6nyh,6di0,3s3i,5omg,5vib,5s89,3flw,4cyi,6tgu,6n9p,6npn,2hog,6yxv,1f3m,3rep,6vxu,6yph,4fl3,5u6c,5ory,6oqo,3bu3,1jvp,5r98,6tei,7a4b,2yn8,3juh,3mh2,2h6d,3qtr,4mwh,6bdn,4ft0,3qkl,4xmo,2gsf,3dgk,1gjo,4cmu,1h1s,5lpz,5o0e,3vw6,1na7,3o23,2xk8,5b0x,5n1d,3gcu,3dpk,1xr1,4ib3,3sxs,4czu,6tlw,5otd,5bve,6fi6,6yti,4wnp,3oy1,4e73,4yjs,4uyn,4im0,3c13,4yxr,1k2p,4x0m,4wkq,6tfu,5vhb,6bku,4eh5,3og7,3pzh,6npv,3k2l,5aab,6ypp,6w8l,3zo1,3hmm,4w4w,6fr1,1fmk,6o8i,1zy5,3at4,7a4z,4fk6,6w7o,1r0p,5z1e,2r3f,5nkc,3p4k,2ewa,4p90,6rq4,3qqk,5n66,4qmz,5r8w,6xx8,5os6,2c6o,5o26,6fvg,5hkm,2xik,5n37,3bkb,4jia,1xbc,2vww,1o6y,5hlp,2wtj,5m55,5i3o,5ut0,6w39,2btr,6ege,2cjm,5e7r,6gjd,1xha,6r4b,3uix,7b42,6q4e,2vts,7ng7,3niz,4dfx,4fnx,5s7m,2y8o,5op2,5o12,5qim,5n52,3a7g,4qta,4d0x,6sod,1xqz,2v7o,4fsz,4ehz,4wb8,7kxo,7nh4,6gla,3ugc,1mqb,4ux9,2uzo,2yir,2rg5,6fha,6esa,5r9o,2bzi,2wmq,2pz5,5s7q,3orx,1h08,5o90,5tq4,6sox,4dce,3tac,5kvt,2hz0,2r64,2vto,5oo0,5nk0,3nax,7kpm,4ivd,3oxz,5av1,5r9s,6c18,5p9m,4iad,7jyr,4gmy,3a8x,5n23,7sui,5te0,6ssb,5d9l,2waj,3vby,6hhg,6tn8,3iw8,3uqg,2oiq,5i4n,5m75,5kup,2hk5,5am6,7b33,2yhv,5fxr,6hex,5a14,6yi8,7a51,2wtv,7ksi,5oq6,2iw6,6btw,3rhk,6o8u,5hg9,6pl4,6cpw,4mxo,6wto,4ii5,4lyn,3fls,1w84,6vxq,6zcr,6y9r,4nfn,1jsu,6zqs,4ans,3fkn,7apg,3ad5,3w32,6oav,5tkd,6xlo,3vs3,5u9d,5ew9,4jx7,6qg7,4rj3,7cbx,1fpu,4dg3,3nz0,5byz,1jbp,6in4,6sq1,1q8u,3ce3,5auz,4gk3,4x7l,4azw,2src,7aya,6rb1,3eyh,3fxw,6ycu,4agu,1fin,4btk,3wf6,1svh,4gv1,5n3d,2ym8,4ztn,6g34,3fmk,6vni,5x2c,3mn3,4bck,4yjo,5ose,5vda,4fv0,6bfn,3sls,5yvc,1fmo,6y4u,3hmi,6yoj,6c1o,6nbs,4i22,1q3w,3daj,3mj2,6wak,5lqf,4cli,3ue4,4zzm,3r9n,3d5v,4dc2,5m4f,5ane,5bue,3be2,3k5u,3cd3,4c2w,3sqq,5nkg,3dqw,6cmm,1lr4,4alw,3qgw,4gt5,3gcq,5toe,3fup,6tls,6brj,4ek5,6mzw,4l3l,3r8v,5xyy,3nw7,1h1w,4a4l,3qwj,3r7u,6ayw,7avz,4fz7,3qrk,6v5n,6ynr,4s31,6ath,3fhr,3u51,7aaz,4ftc,2c5o,5s7i,2p33,7ab1,4qte,2xuu,1ove,5vc3,5fdp,6q4a,1y6b,4gub,5c26,6rsc,5e1s,5r9k,1luf,2ydi,5ur1,1w8c,3zxz,5dyl,5d1j,5n33,6g3c,2c3j,6q7e,5gnk,1vyz,6i2a,3aox,1y8y,5kgi,2baj,2c6k,5os2,5e8u,3c1x,3cjg,4iwd,6kla,3biz,4hnf,3miy,2wqo,5cu3,6qty,6g9a,4k9y,6snx,5kmk,5w85,5m51,6mm8,6n78,2yjr,5ut4,7q7k,4fod,5h2u,4u79,2o0u,5ng0,2xnm,1oec,3mdy,2ofu,5izj,6cn9,4deg,7jxm,7l26,5iui,5ol3,2y6o,4i3z,6r6e,3c4f,7be4,7q8w,5fgk,5jfw,4krd,6sde,2qo7,2bik,5j8i,7b34,5i9v,6r3d,1di8,6q3c,4ivc,6hvf,5vd1,2uzt,5r9t,7aw2,4iac,3upx,1wcc,5p9j,2xrw,5jrs,5eho,5iis,5s7v,2b1p,3tiz,3wzd,3vid,2vnw,5cf5,2vth,5yk1,4qye,3brb,2w1h,5grn,5nk7,2xbj,5n3c,7orf,4bfm,3q6u,5tex,5usy,3fml,4u5j,4pv0,6g33,6di3,4dh7,6cqh,6eh2,5ku8,4wnk,3qrt,5o2b,5jq8,4loq,4otq,6cdt,4rc2,3dxn,5toz,3kxm,6y2o,4x2j,3rni,6g91,1xh5,6ru6,6tll,6bru,1yi4,6c2t,6i83,4gk4,4x7k,5m5a,5tbe,5xqx,7bjx,3fjq,6x3n,6nvh,3ekn,5ei8,7akg,3poo,2f7e,5s79,3rpo,6y6v,4e93,3mh1,7cja,4rx5,3qtq,3bz3,6s90,6ziw,5orz,6you,1y91,3qam,6vov,4fi1,6bqq,4ccu,5cvg,6vph,6zcu,1smh,4afj,6ypk,5mrd,4aot,6lnm,5a3x,2gng,5t6a,6yqk,6tfv,3zc5,6m9l,4l9i,5nwz,5bvf,4k33,6vnv,4bkj,6dd4,3fzt,4yjp,3pls,6hm6,5osz,5tob,5n1g,4wsq,3gcv,4qp4,4ib0,3iok,3o71,5otg,5ra8,5mty,1zz2,4two,3gni,3eqi,1h1p,5lpy,5vuc,7mxb,4zsl,4lmu,6gu6,3oz6,5vnd,6qj7,5w9e,4bhn,6zln,3qqh,4bzo,6hk3,3h9r,3dko,6pk6,3q5i,4xrj,4d55,3zo2,4fv7,3v51,6unq,7olx,4ez7,4eh6,4obq,6npu,4b4l,4anl,5hx8,5aaa,6yps,2xyu,3gc9,4ae9,6fng,2okr,4f9c,6r4a,3zsg,5y90,5cu4,7b41,6jpe,4kba,5kml,5m56,3zly,4foc,5ut3,7q7l,6emd,4gva,7jxu,6q7b,7r9p,5n65,5ml5,4qmy,4ieb,1re8,2c6l,5os5,7kxl,6glb,6rsd,3c0g,5j1w,5ikw,2yiq,2rg6,2wel,6fhb,5r9l,2bzj,4fsy,5dyk,2ycs,5cy3,5s7n,5o11,6pnx,5qin,5n51,5x17,5xp7,4kkg,5zj6,2ojj,4p4c,6q4f,2cch,2c0i,2vtp,5vc4,5wg4,6spy,4gue,4qqc,1ke8,7jyq,7suj,6gva,5li1,5vd5,7kxp,6no8,3nnx,3mgy,5av2,5r9p,3bgz,5ct0,2vtl,5oo3,3cly,3nie,3bhy,5nk3,3nsz,7aj4,7dhn,5s7r,5c01,5tq7,2b9j,2ds1,6fjb,4qna,7ksj,5oq5,6gue,5zn3,5ap7,2x8i,6jux,7a52,4ptg,7p1l,3cpc,6hme,7b30,7k0v,5fbn,5eko,2io6,5fxq,4au8,3tud,6fdy,5f4n,2jc6,5jfs,3el8,7r9l,3pxk,4umu,5ouc,2oj9,6qg4,3qtu,5nqc,4gg7,4b6l,4gu6,5opb,4ft7,2oo8,7m0x,4qt1,6so4,3ad6,3ti1,4g17,3qkk,3fdn,4l8m,3mb7,4w9w,6vxr,6vpl,6zcq,4nfm,1jsv,4bgq,3f2n,6e21,4ks7,6vgl,3kmu,6vnj,4dh3,6f26,1rek,6anl,5osf,4yps,3fhi,6qa1,3wf5,6em7,5n3g,6n0q,6g37,4yom,3fmh,5auy,3r8m,5n4z,4jt3,4dg0,3ma3,4x2n,1r1w,4ix3,4i93,5vja,3p0m,6xvk,5nkd,3jpv,7dh9,2jed,5uga,4clj,4zzn,3qql,3k5v,3r1s,4ez3,4eh2,2exe,2uw8,3ewh,6u0k,3mj1,4fv3,6hd4,3cy2,5m6y,6y4v,5mmf,4bcp,6oph,2qod,4s32,4yjt,6nfi,3fzp,5l3a,7aay,1u46,3r7v,6vql,6m9h,4iz7,3jvs,3srv,7b6f,5fg8,7avy,5uad,6d20,3r8u,7oox,7ltx,3rcj,1pxo,6gu2,5ih8,5lxc,7bjd,3q4u,3bi6,3hko,5yjz,5ukf,6tlp,4ek6,4crl,3lm5,4o2p,2pvf,3fv8,3zbf,2ydj,3mpa,2in6,6raa,3eh9,4e6c,2yak,5r9h,2wmv,4rmz,2vtt,1q99,3zze,6q4b,2pe0,5h3q,5bx6,4knb,4m68,1y6a,4qyy,6hny,5s7j,5op5,7ab2,4i5c,6fjz,5mo5,5dls,4qny,5hlw,4fux,4yr8,5bq0,5dhj,5cu0,4fbx,4jqe,2qg5,6i2b,6slg,3r28,7ll4,5os1,5o21,5e8v,2cmw,4qrc,3n9x,1zoe,7jxq,3myg,3c4z,2z7l,2c3i,2o2u,2yer,7r9t,3zya,6q7f,4iaf,6kzc,1ke9,1ung,3ql8,6q3f,6no9,7kxq,5vd4,7nr5,5av3,5r9q,1vjy,4fkg,2c0t,6rfe,3oez,6p8e,5hhw,7oy6,5nk2,5tt7,3orz,7aj5,5s7s,7ax4,6sgd,3bwf,5tq6,2npq,4rfy,4l68,7ksk,5ap6,5ot5,2qo2,2py3,5fbo,7b31,6hmd,5kbr,3bqc,4ag8,4iza,5j5s,2zdt,2vwi,4j95,4umt,3vs1,3h9o,5mjb,7l1x,3g9l,6vhn,3gxl,5ugx,3fkl,6qp5,3fqs,3flq,3up2,4jr7,7c3g,6zcp,6vpm,4anq,3mb6,6ypn,3e3p,4zjj,6ra7,3bu5,3gen,6oqi,6es0,6ygn,4wov,3ddq,1phk,1fvr,2hyy,5x2a,6vnk,1bx6,7a2a,1rej,5n3f,3krj,6y8h,6cfm,3r7o,4aoi,3k3j,6em6,6acr,4ztl,3o50,6g36,6n0p,4x7n,3r8l,5aux,3iph,6t2w,3ekk,4j52,5nxd,3kxh,6fn5,5otz,3zs5,6nsl,1q8w,4i92,6db4,6tew,6xvj,3pxr,1jkl,5nke,6wiw,4zzo,6bln,1hcl,2f7x,4px6,3rpr,5ang,2uw9,5omy,6bql,3vc4,4eh3,4fa2,4bgh,3ac2,3cy3,3ezv,4fv2,3uo4,7nrb,3n51,6y4w,3raw,4bcq,6vns,3qri,7aax,3vo3,6nfh,4yju,4s33,3dzo,3krr,1uu7,3uc3,7avx,6bbu,3jvr,7lty,6yvs,4uak,7bje,5ih9,7opg,3gcs,3q4t,6lvk,7a5d,4ib5,3efl,3ion,3ubd,3lfa,2ydk,5fto,6fex,6gvx,2yit,5hor,2wei,6eix,6frx,5r9i,2wmw,5dfp,2pe1,6d1z,6q4c,5hzn,4r1y,1oiy,5bx7,4ifc,7wf5,5op4,5s7k,4fta,6ekd,5qik,5wp1,2bpm,5mo4,2xnp,5kmi,5m53,4xv9,5ut6,7q7i,2y9q,4fuy,2wqm,5kzi,5n93,6gjb,3odz,6r4d,7bu4,7b44,7ll5,5k4j,2nru,3tjc,6i2c,6qag,3ocg,2c6i,5os0,6ema,5kpk,5xd6,7jxp,5xv7,5ar2,6q7g,4izy,6r6x,6pjx,2vgp,7siu,4d1z,3w2c,6qyx,4i4f,7jxl,5h0h,1u4d,6jwa,7q8v,7be5,2z7q,5jfv,6qdz,6ac9,5iuh,5hti,5tr6,5hnv,6sdd,7b35,5eyk,5i9w,2fo0,1r78,2f57,5vd0,2uzu,7qgp,5ci7,5icp,4ivb,6q3b,6smb,4h3b,7jnt,5r9u,5dnr,2brm,7s1n,5k5n,2o3p,5p9k,6tu9,7aw3,7jyt,1oky,5s7w,7dhk,3wze,6gcx,5yk0,2vti,5cf4,5v82,4puz,6yr9,5n87,5nk6,1y57,1pmn,3my5,6cth,6fd3,6em2,5n3b,5lmb,4zth,3fmm,3qru,4bcm,4gs6,3rak,6v5p,6eh3,4lop,7b3z,5o2c,6qa4,6wxn,6qs5,4x2k,7lqd,4nwm,4rc3,4ix6,1xh4,1how,6ru7,2e2b,6aaj,3le6,4x7j,6i82,3q9w,6zwp,6nvi,6qy7,6x3o,3eqp,4cmo,2fvd,5s78,6bdl,6so1,4x6r,3r1n,4ump,4yll,3s0o,2vn9,2erz,4qq5,3we4,3mh0,6vru,3kck,6yzh,4uxl,3fsk,4cfu,2ya9,3qal,6yot,5cvf,6bqp,1w82,2x39,6ypj,6vpi,6yqj,6ubw,1uu3,2gnf,3elj,2f9g,6tfw,6obl,4a9u,6ynt,6mom,4yjq,4oth,6k77,6hm7,3oy3,3qup,4gt3,5n1f,5otf,6mzq,6nsp,4ek3,3lm0,4ib1,4pf4,4l3j,6aar,4twn,3r8p,3a62,6y7w,5mtx,5ra9,1pxj,6fq7,3qxo,5vub,3eqh,4uzh,4o6l,4l7s,3r9h,6fj0,4bzn,6v6l,1fgk,3qyw,3rpv,5vcz,6bik,6s17,3op5,3ezr,3zo3,1gii,1jlu,3hmo,4bbm,3dls,6wtq,6npt,4obp,4eh7,4i24,4ckr,6bkw,4anm,2xck,5m06,6e4f,6fnf,3gc8,5j7s,7b40,3vrz,6dcg,4eqc,3vhe,5kmm,5m57,2w5h,3amb,7bb0,5ut2,3zlx,4e5b,4fob,6jmf,3npc,1r39,2vwu,2c3l,5ui0,1xba,6q7c,5r8u,5xs2,6vn8,6jrx,1v0b,2bal,5n64,5os4,2c6m,5e8s,5v61,1rw8,7a22,6rse,7kxm,5r9m,2bzk,4xg8,4iaz,3lfe,5s7o,2ycr,5n50,5g6v,4k0y,3rp9,2vtq,5vc5,2v5q,3pj8,3oef,6q4g,4jxf,4dfz,6spx,3g0e,2w05,5n9k,5wno,3kxg,1p4f,3igg,5y9m,6vvg,3g5d,3gfe,3rkb,5auw,7bjr,2psq,3fxz,6n7b,3e8e,7nqq,7akm,5n3i,1sve,1pme,5nhv,6di9,6g39,6gr9,2ym5,2c30,5o7i,2rfs,5wal,5d41,2vz6,7b3q,5orp,4ouc,4xoz,5tiu,5n7p,5r91,5lvn,5s80,3i7b,3say,5mhq,3r6x,3hrb,7apj,5c8n,5lcr,4ft9,4ff8,7axt,5n5l,3kfa,6nze,5cnn,5oor,7btt,4xhg,2xj1,2hel,2xiz,2uvy,7dtz,3uyt,3vbt,6hhj,4rvk,2xvd,5htb,3ri1,4ap7,6hwt,4i6q,4y12,4z83,6heu,2zaz,3lxp,3cbl,3l9p,4rqv,2xkf,6i5i,3d15,4j8m,4c35,4f1o,3r02,4hys,6l22,3zdu,6guk,5iha,5ug8,6qxk,3fc2,3e92,6sgk,3qc4,6sou,4hpu,4xw6,4i0t,2oxy,3uzp,3zrm,6hkn,3d83,2qi8,4d5h,4ub7,3cqu,3v5l,3uol,4zp5,6l16,4m13,3nnv,4iai,3v8s,1ke6,5g1x,1unh,6zc0,3acj,3nyv,6y80,2bdf,5h8e,4hvh,3cok,2oid,4yo4,5kgd,4qms,4nj3,1vyw,4rll,1yqj,2biy,6qah,3fz1,5e8x,4aw2,6fnm,2o8y,3s95,4p5q,1nvq,4o21,5imx,6sfk,3w2p,4kbk,3rk5,4hct,4i5m,5s7d,6hnw,4eon,3vvh,4ftn,4h1m,2uue,2yfx,4fkp,1q97,6gqj,6bs0,3pj3,3owl,2w1z,6yz4,6sps,4xh0,4r1v,4m66,3l8p,3v5t,4uj1,4v01,6ng0,4fvr,2owb,4kao,6yg6,4xg3,4h3q,4a07,1zys,2wmx,2a2a,5r9f,3lfn,6qmo,3vqu,1yol,6few,4xp3,3ttj,7ccu,5n1m,5ajq,2b54,5n9s,2pvh,4ek8,7nth,2izs,5o5m,6ylc,5ra2,7oov,6mwe,3eqc,7ack,7bjj,2p2i,2jdr,4fg8,4yhf,5w7t,5n3q,2gfs,7vdp,5lwn,5uit,4js8,3pix,2wd1,4mkc,3hvc,5wij,6ate,5osp,5fp6,6tpd,1k3a,6x8f,5orh,5cau,2br1,6c1b,4bbf,6y4x,2uw6,5vam,5mhi,5lcj,5ia0,7ajm,6nec,3dnd,6i99,5t8p,5mot,5tco,5x1r,2ac3,4asd,6xdd,6wly,5ouu,2r3o,6vrf,1oi9,3roc,5mpj,3flz,5s84,7jy4,3hrf,4ujb,5csh,6aua,5r95,6occ,4tnb,3kvx,1r0e,6bab,7a4o,2pwl,3i5z,3itz,5ack,5tts,5s77,4asx,1cm8,1pye,1pkd,5k72,7jv7,5moh,5hd4,4kb8,3q9x,5ei6,6qy8,6w3c,6ru8,3pyy,5otq,7kl1,3i4b,3sxf,1rjb,5a6o,6cqf,6ync,4el9,5osl,4mta,4w8e,6cnx,6y8c,4xyf,2gtn,5n3m,5cep,2uv2,2jkm,2i1m,3owp,6gcw,2vny,4y73,6h0u,4fkl,3pp0,3hp5,5nk9,3dk6,5s7x,4ftr,4eor,1h01,4e4m,7khg,1vzo,3bel,3gu7,6f1w,5jga,3fl5,3v8w,5aa8,5qtz,6szm,1okv,3r63,4g6o,7kxz,4ewq,6kmh,3fi4,4e6q,3lcs,3u4w,6l12,5r9z,5hoa,2brb,3tkh,6z54,6fil,6i2p,4gii,4qmo,3nuu,4jdk,3zfm,3oct,5i9x,5eyd,3uto,3cxw,5h0g,4dei,3byv,7q8y,3zcl,6m95,3pa5,6q7t,3vjn,5iug,3tzm,1o6l,5yu9,4qpm,3m2w,4eyj,3uim,4jbv,4fkt,6q4h,6tw2,3g90,1oir,6spw,5hze,4eoj,3ik3,4ftj,3ori,5ehy,4euu,6soi,3a7j,3cth,4fsw,4fih,5k0x,4wb5,6elr,3v5p,3c0i,3lck,3zos,7kjc,5r9b,2bhe,6yg2,4xg7,4wg4,6eis,5r8z,3mfs,6i2h,6z44,6ehk,4qmw,3hl7,3l9l,3lxl,4fmq,6qal,1ckj,3r73,6bp0,2vwz,5etc,2yex,3wik,1p14,3x2w,6sfo,3zlw,3qu0,4dgm,1j91,1ydr,6ya7,6fni,3gc7,3dj6,6pxn,4nw5,6k0j,3zsi,3en6,6g9h,3pze,2e9o,7a6k,6b8y,6tua,6lud,5hx6,7oai,5mzl,4gw8,4anb,5csp,5orl,4ctc,4fv9,5l2s,5lar,7olv,6z5c,5ho6,3pxy,6xva,5zjw,5upk,2xp2,4wrg,2r3k,7dh3,5ia4,7mck,6ble,4u3y,3huc,3qqf,4aaa,5wjj,2ghl,3rpy,3r1y,6y7x,5ra6,2hiw,6e99,4yzc,2jdv,5o8v,5lpw,5x5o,4n6z,6ft9,5ukl,5oti,4c3f,6brc,2vo6,2pvl,2jii,7nns,5win,6ytd,6vnx,2qon,7b3m,6mob,1mp8,3p7b,5nhj,2gni,5hq0,5odt,5s85,2e9v,5cvh,5vlo,5e92,5n7u,5ndt,5dn3,5r94,4b9d,3heg,3rzb,3d7z,3f5x,2r3r,2w96,7bko,6thz,5s76,5cqu,7e75,5x8i,3q9y,3ptg,6qy9,6nvg,2jdo,5n9n,3ms9,7atv,7kl0,5otp,4dh8,6ynb,6ccf,3ag9,4ona,5osm,7b3t,5n3l,3r7e,6z1c,4w8d,5xdk,5ceq,4y72,6a32,6q4q,4jbo,6rfo,3dk7,5dia,5mp8,5nk8,1ywr,4dfl,4qqt,4i5p,3pg1,3u6j,4e4l,1h00,3orp,4ll5,5s7y,3gu6,3wzk,3kn5,1ig1,3fl4,3e64,3lfs,3vqh,4fsn,3ctq,2gu8,4g6n,4geo,5aa9,5i8a,6gvj,6eij,3bgq,4r6v,6z55,3tki,6l13,4qmn,4gih,4zy6,5i9y,6ges,4jdj,6gwr,4f6w,4deh,3pa4,4y46,6hrp,6gzm,1wbt,3vbq,5jfx,2xnb,6yl1,4gcj,1urw,6fyp,3uvr,4c61,6hor,7ree,4nm3,6jol,4equ,7at9,5ime,7a49,2oxd,6q4i,4fku,6te2,6gqo,4ith,1m2r,4i5h,3fy0,5yf9,5s7a,3zep,4cd0,4ftk,1w7h,6jqr,5x18,6jkm,4kkh,4fii,5vi9,5s8b,4ehv,3tnp,5kcx,3aqv,4at3,3qd4,3h30,6hdp,1q61,3ckw,3v5q,4v04,3c0h,2cdz,5k5x,6eir,6yg3,6e2m,4xg6,5ts8,5r9c,4qmv,6eru,3mfr,3l9m,6r3s,1ql6,2f49,6y85,3byo,6hzv,6jxt,3x2v,1xws,3e87,4lm5,4rqk,6pxo,6ya6,1yds,6itt,6fnh,4ae6,3vhk,3zsh,7a6j,2z60,5owl,6npz,4eh9,4ccb,6yjc,6o5z,3ac8,4y0x,4ctb,4fv8,5cap,6z5b,4nka,7auv,1qpc,2r3j,6sp9,2hwp,7nxj,7t4n,7m0k,5ia5,2ghm,3qqg,3hub,6fc8,5ra7,5t1s,6y7y,6yvy,7bjo,4ceg,5n1h,7opm,5a9u,2xk4,6ft8,1jpa,3kxz,7a5n,2pvm,2vo7,5u8l,2jav,5oth,2qoo,6z4z,6obb,4m0y,6vny,6yte,3p7c,4otf,5osu,4txc,5n3t,7vdu,2gnh,6tfy,7nvq,5cei,5kz0,2qhn,5w5q,1q8y,7kl4,1qcf,5auv,4bie,5n4u,7aym,5oqu,7akl,6n7c,3soc,5d11,5n3h,2ym4,6g38,3f6x,6gr8,6yty,6vne,4c4f,2f4j,3eha,3f2a,2o64,3lq8,5hg5,5r90,4mxc,4ks8,4ynz,3i7c,3idb,6bke,5s81,5lvo,3rmf,3h3c,3hrc,4w9x,4tyg,2zb0,5vfi,5l8l,3dfc,5n5m,4zeg,4f09,2fso,5oul,5ctp,5cno,3qtz,5ttv,4gu9,5h0b,3bys,1wbp,6hrt,2uvx,6yt6,3hv5,5htc,1v0p,4m84,3t9t,4ot5,6hwu,6qaq,6het,4nm7,3d14,6i5h,5drb,4gfo,4c34,3py3,2c1b,6qfl,1bmk,6l23,3t3v,6fck,3qx2,6g4j,3uli,3ort,3e93,1q41,5ug9,5tq8,3q04,4hpt,1i44,6sot,4g1w,6gcr,3zrl,2oxx,6dbm,4fki,3bhv,4hgt,3h10,1ywv,6iup,2xba,6s1j,4n70,3dk3,3gb2,4y85,4ct1,5yv8,3zon,4tt7,6l17,4m12,3nnw,6pdi,2brg,1ukh,1yxu,6z51,3wbl,1ke7,6gip,4hvi,4rss,6y81,4gvj,6gro,4z55,1tki,5etf,6fiq,5kge,5e8y,3sw7,3js2,4i6h,6fnl,6pjj,5k3y,6kyq,6g9m,6fyl,4hcu,5t18,2w5b,3w2q,6sfj,3jy0,4eoo,4fto,5s7e,1lew,3kf7,4ejn,6gqk,6xl4,3c7q,4fkq,4m67,1ywn,6ol2,4hgl,3kq7,2x9f,2vag,4f7s,3pe1,5r9g,6yg7,4kip,4a06,4h3p,4xg2,4rwj,1dm2,6gih,4xp2,3qd0,1z5m,5n1l,2b55,7nti,5otl,4zly,2vo3,7dd1,3r8z,6u6a,7oow,5ra3,4fg9,4zsg,2jds,2p2h,2vx3,1uu9,3nx8,5qu0,5nho,2rku,5n3p,5b2l,3r7y,6ncg,5uiu,5cem,5l6o,6yta,6sd9,6obf,2qok,5ek7,3pvg,4ypd,2etm,7baq,7kp6,6x8g,5m6v,7ols,6c1c,5val,5owh,2uw7,2i0h,6nja,7chn,7oal,7bcm,5opu,5lck,5ia1,4bzd,4ase,3rjc,5x1s,5bui,5ani,3dne,1pyx,6mib,1kob,6wlx,7a4r,2r3n

==> trainval_codes.tex <==
4oex,4mhy,5m4u,5il1,5uxo,4orx,4csd,5x4m,2q2n,5aqh,5da3,3ery,6vue,2xe4,1szd,5jo2,5g11,4n5d,5wdk,2qpj,5y3i,5l6p,2oi5,7qk5,6cqd,2r5t,5n6n,3qrx,2jfp,6nfy,6n5x,3dxb,5nps,5mks,5kh6,2xc1,5y1u,5u0i,2pvv,2oq6,2o06,2yb0,2j7m,6kmj,5li9,4phu,3s70,4k2p,5mm9,4rmj,1zkl,4oj4,1w0n,4pmt,5ow8,1sw4,3d27,6g5u,5fsc,4dkp,3tiv,1y3p,6d1k,1p57,1y6q,7op9,2ri9,4gnv,3m2u,3rc5,3mvt,3awh,3zds,1k04,6b67,4mn3,3axk,2y6c,6mj6,1wpv,4lj3,2wva,3hd3,3ir2,5fjx,1kh7,4ln2,4phm,3gw1,3wxl,4ob2,6k3l,4ezt,6pii,4k7i,1sm3,1uti,3bju,4x15,2ogy,4eoh,3s54,3kf0,5kdf,4oz1,3v2o,1q91,4pop,5wg8,6ful,4al3,4r8v,6qfs,1a7t,3cmq,4j8s,4lh7,1ro6,2vpe,4od7,6hoi,1n2v,3kr4,3mkn,4kep,1lkk,2hf9,4glr,1ugp,2ymd,5n69,1z1s,4wn0,3lpp,3v4j,4piu,1gkx,2yc0,2ou7,2hzl,5tci,2i2s,4zmf,1gny,6n3e,4go9,1fxx,5n7n,3mo8,1jlx,6okg,6apz,2j9n,2g4l,5mzn,5t7u,5dx0,5kj2,3d3x,3kze,7mel,5y3q,5w2s,5tzr,4myd,3kme,1dic,2jfh,2dww,3pyc,2jau,6ueg,6w3y,6o9b,7jg4,4axd,6x1z,4onf,3r7b,3rvb,3wf9,5ahw,2xi7,2ixu,6ttg,2fxv,2haw,2fmj,2hvw,6tld,1al8,5ofv,4yec,6xef,7m5u,5v8t,6usc,5vtk,5afl,5m4q,1xk9,2q8h,5bro,5o3r,5yvt,3pee,3qsd,5whh,2ww2,2we3,5xzj,6vua,6eji,5n49,1tlo,3uvu,6me1,4mv4,4dur,1l2t,4m74,6euw,1ork,1qk4,1alw,3lmn,4f1m,3tbh,1bpj,4u82,3lpl,1nki,6i7w,6ewk,6fdu,3npr,4wq2,1lyv,1z4n,3n1r,3ga5,4z46,4j3u,6hip,6n94,2bmz,3bxh,1ocn,4gwi,4qip,1tok,5fcz,3mok,3s87,1ht6,3tvl,3gp0,1oss,6jfm,1nzl,5pwa,6sgi,6i0r,6rbi,4fut,5jaz,5jid,3qu6,4kov,5dhf,4ixh,4lz2,3fu0,6yn2,3r24,2ody,5eyz,5jyy,3t4p,2wic,3rv5,3loj,1atl,1w8l,4qsw,4x11,4af5,2wzz,4n57,3fa4,4nq6,1lov,5o48,3tdu,4r9j,2iv9,6eqv,1fo3,4gxr,4kqp,6e8h,2xv1,6mod,2qbw,5nzm,2j0l,5bnm,1j4g,3hnb,5l9o,3h8b,5bqs,6mia,3gxy,5l0i,1kec,4o1x,1pdy,4lny,5t2p,1ln8,5tzo,2wl4,1d2a,6kl8,6zjz,1rzx,5km2,3eyf,4o7d,5oqw,6fn9,4awf,6g98,2oc2,5u9j,6bae,3ll8,2r3t,2ews,3sfg,7l4u,2zm1,2ebo,6bkg,6m8e,6mye,6bcy,3q7d,5c2o,4yyx,3rrz,2a25,6poq,2yjd,5izc,5my8,4pfk,6gxw,5ot9,4ijp,4my6,6p6r,1a0t,6rrm,3nps,5enc,5i5x,4cc3,4zg6,4fai,7qjg,4g6h,1pl1,1fh7,3ugq,4bb2,6izq,3nfk,6jaq,6quw,4f8j,3pp7,1so2,3uwl,1twi,6g5p,4v26,6os6,3rx7,4d1j,3blu,1l7l,6f8n,6hgr,1dy4,188l,1csn,1ej4,6ppw,5iee,3l6h,3cwk,5zc9,5yj8,6o94,5eqe,4pip,6fvm,3w5n,3rv4,2bvd,5vr8,4eih,3u1i,3id7,3u9w,3ncr,3nqs,1utl,1ir3,4p3w,4ewn,1qw7,1ga0,1low,1onh,2vnf,3zzh,6hyt,4dnl,4k5p,3k05,3b3s,5e3a,6k4t,1jt1,1odj,5tri,6afg,4zkf,5ey4,5c3o,1fsg,1yn8,5w7w,5tei,3qwd,4y4g,2oa6,4und,6mxe,3rcg,2xn3,2psj,2vj0,7d23,2bf6,5ybi,6nsx,7rr4,5otn,4csy,5m9w,3k8d,5c0k,2w47,5x9o,2hrw,3phc,3d2e,5oht,1gia,1k3b,5umn,3gez,4nyf,6way,4yia,1kbc,2idj,2oo1,4qf9,4b3d,3ti8,5qi4,5wbo,5uxn,5ujo,1q1y,6ig8,5mxk,4b6e,2ifv,2euk,5lsh,7pc3,7nws,2pgr,2h4v,5m2q,2wi1,3m89,5sb0,5lwq,5mlo,1w49,4yje,1d2e,4du8,3rnd,5npr,3fgc,2jal,3pce,3s9e,3i4a,1gox,5o0s,3c39,4ido,1y1m,1lok,6iht,2vdx,4cc7,1mai,2aqb,4mz6,3clp,6hcw,6efk,3aaq,2xxx,3nss,1lhv,6om4,1uwt,6jon,3gk2,1lin,1j14,3c6w,3lmk,5vb9,2okg,5d6e,3w2o,3s45,4ce2,4igk,2xsb,3rl7,3a1t,6i7r,3ukr,1t0h,3pa6,5etx,3b5j,3cpj,3ocw,1mpl,1ga4,6qzh,4phl,6yg1,1x8j,5yi8,3iv2,1a4q,4x14,3mph,6fwq,6jdl,6o57,6r0u,3ozt,1tet,6f9r,5d7e,5w19,5u99,1hn4,6b27,6gqm,4fci,1t3t,6c67,3ru4,6spt,3mam,1l2i,1pu6,4rqi,4r0i,4tz2,4lh6,4j8r,4pfw,1nli,2cjc,1urm,6y74,2zyf,2z8f,3ip7,3pf3,3tuu,7jxx,2hf8,4keq,6ghv,6ox0,4rlk,6ehh,4y93,6tq4,5o1s,2j6l,5ugh,5oxm,4u3z,5xxk,2nq6,3b69,5vcv,2vf3,4o3a,6bsx,1htd,3p1d,2bo4,5nqr,6qw8,2bw7,3rwg,4tkx,5mah,4cpy,6wue,6gh9,1f7b,5bvk,2rio,1j1c,1li9,3iof,3i4y,2vo5,6lsb,5mtt,3q9c,4bae,5yum,3ipx,2ycm,3ozg,3liy,6n69,2b1v,3t2c,4dcd,2gz2,3omg,5t54,5yv5,5icw,5li3,5av0,5ad1,3m4z,1z8g,4gzx,2ydp,3zjb,7ul2,4lj9,5za2,5ful,3hv8,1rm8,2yhw,2hv6,4p5e,2oym,3uie,3thd,4q4d,5irr,5jal,5lx6,1kzk,4upu,5lsc,4z1v,4ncn,3hmp,6fh3,3q2j,4ojq,1m51,5yid,5wey,2q8f,3ksq,1pvn,5m3b,4clp,5l8a,1jfh,3q8h,6zvo,1pym,1xa5,6tel,4i07,4uwh,2pwd,3uh2,4nds,3kpu,3g0i,1ikp,5ofx,4oak,2hig,3kut,3ud5,4j51,3dzt,3hii,1f2p,6y0u,6ubh,3q6s,4ufm,6t5i,4uns,5o7e,5ove,4tor,5yec,4i72,6h77,4ctk,4v0r,5v7a,3hww,1jlr,2qta,3fdt,3nq3,3gzk,3kiv,3l21,5vnb,3exi,3fci,3e9i,4xmr,6zdv,6ahs,5mxx,3rup,4m6u,3td4,2g7b,5mka,4bvn,4qp2,1h4w,3qxh,4usi,3sov,3jyr,3ecn,1gpu,5w7x,2dua,5wlg,1tq4,2eqa,2e0a,6opj,3qzt,4w5j,4kr5,3ess,6buv,2vkh,2ykk,5op7,5ivs,5e6o,3zhf,3u3z,3uzd,5kam,2wji,2clm,3oxc,2ozq,4iic,4rrf,2bws,3mbb,6f7b,1uod,4glx,1bob,2j83,7a74,2ves,3wca,5lz2,5f1u,5ul6,1z6d,3ry8,1t7f,5i3j,2mat,5duv,2a3i,5bv3,4to9,5ixt,5vm5,3p79,1yfz,4kmx,3b8z,5ah2,2z7r,3otx,5d6j,4kxd,4h0e,4kpz,3b7y,3chf,2oni,2ypp,5c91,5khw,5x54,1bmb,6qfe,5up0,3omc,2bgr,6pyb,4inb,5nn4,2b1r,3fl9,3upz,4p6e,3lka,6h7d,6hde,3ckb,6z58,4bb9,5km9,4rt0,3kgq,2of8,4py1,1icj,3gkr,1fkw,3kjn,4du7,2q3x,3rtt,3r5t,4qj1,4b7r,1r1q,5lub,1ux7,6cck,6f20,1uj6,3v43,4u8w,2rkd,6zbo,3o57,6bcr,4lyk,1bt6,4pz5,4o4k,3fai,6fh7,4aci,2d0d,3r3q,1qji,3cl0,4rx7,5m1z,6cen,6zsj,5cqx,1kjr,2i7d,6pf3,1s9v,4h12,3dnt,6z7k,1ppw,6pg3,5wqa,3vw7,4ual,1dqn,5a1f,4b7j,3mi3,5zkc,6ckm,4r74,3keu,3bf3,5osx,6tkk,1g3m,6hm4,3pdo,3rdq,3qmp,3ax2,4wcn,6hh5,2pnc,4oyt,4b4n,6agt,5a7c,1fmj,1v16,5wre,3juq,2p6x,5i29,5ugg,3icn,3qck,6f92,3ta1,4m3p,5wxg,2q7y,4nan,6iae,2p02,3u8d,1nte,2vwv,5foo,1s89,6i0x,2wfj,6exz,5jin,2dw6,5tg1,1zea,3uha,5sdm,7khs,4dcx,5xp5,5g6u,2i80,4gmd,1tuf,5q0o,1luc,4hry,1yxd,5duw,1m1b,2vhq,7dkm,4jdf,4kwf,4qhc,3aje,3npy,3pa8,1x9d,2iw2,2v1r,1a7c,2o8h,4ekf,3ove,2y5h,5d2r,3t7g,2vyt,2hh5,2gh6,2p42,4pre,3ckc,5icr,2v2v,5vd2,2z3j,6jsz,5tjx,1jgu,4rt1,6ydl,3h5n,1e4w,5tpg,2psx,4uau,3eqr,4a6l,5v9g,5vjf,1gui,4zyu,4i67,5ymx,6gw1,1nq2,4c4n,6ouv,1pml,3wf2,4x0u,1d7j,4cpo,1b57,3c52,7w2x,3qlq,1lp4,6zyi,4u1p,3pen,1rdt,6ra1,4nku,6cjl,4nyt,4j93,6xvt,1nw7,3p9l,6cwn,5x4b,6ko6,4y2p,1kxr,4zro,3dnu,6f05,1jgm,3hfw,4usl,3pnl,6zht,2fhx,4oav,4r75,3pdn,1dil,4b5w,4x8s,6ph1,5nzf,5qu8,6zxi,3tg5,1w90,4fz3,3zc6,4iz0,1gwm,4uui,4l0l,2j9a,5vad,6m8w,1nu3,5w6e,2rje,6hv2,4ycu,4zbj,6xdm,4umj,5cfa,1fpi,3kyn,3pot,3fcl,1jnk,5ws3,1ogd,1uxa,1ltz,5h5s,6y89,5g0q,5hyl,5d9p,6gzy,3hf8,1l7f,3ip9,5xn2,6pxc,6uh8,1pu8,2a4m,5m04,4pfy,2o1v,4k5z,5ly3,5k7h,2qv7,7rct,4r3c,2w3o,5qto,3cyz,3cqd,5cs2,2o4k,4uz9,1wdy,4itx,3ozf,5jzj,2woq,3qq8,3oex,4poc,3nif,5tt5,2buv,6jtc,5icv,4i7d,4hzz,5eou,3b9g,4geg,5m24,4lj8,5wi0,4np9,6eux,4qpd,4c38,6ze8,2uyw,6hoz,3cc6,1m01,1i6k,6ygl,5yie,4pm0,4l0p,4y5i,1d6v,5v5d,4v2w,6m7h,1rql,3p9h,4zek,1h5v,2geb,2an9,1oh4,2w08,2r2b,4bvw,4amw,3le0,3lw1,6d07,3qpo,6yvi,6jb4,4odk,6mmo,3pnp,1gxr,4usp,3hav,6fv4,4x8o,4ufl,4xtp,3qrs,6ia7,3gvu,4lov,3vu6,6bto,3iaw,6h76,7usz,6yuu,1lo6,4zun,3og3,3exh,3i8t,5oxg,6mdq,4eu3,4mzk,4kc1,3al3,6su0,3c72,6xlw,6g86,6nzp,1ecs,3td5,6s11,1ext,4ymj,6nsv,1ad1,3qpw,6o3w,1g1t,5o0a,6whm,1fiv,4dw6,6ew3,5h09,2os9,3rik,6y5m,4bcs,1pzp,1ssq,3jsq,6hm1,6qi4,3fzs,5svi,2vcw,2o4s,5yf1,3zzf,6e5x,1c3x,2yiv,5cs6,5egs,6hay,1cxz,1lbf,3t5g,1lpg,5m34,1l9y,4rrg,1oba,1l8a,4yo9,5dgj,1ew8,1lna,5ws7,6rze,6ppy,4pnc,1i58,7yy3,1yid,1bra,5izu,4e5d,5rdn,2wyn,3max,4qbb,4j8g,2oyk,5f6v,2pa5,1hj8,2rc7,4kmz,7d0q,3ocz,3n5c,2hb4,5uz0,2vvt,6f6d,2h44,5x62,2nyr,1blx,5e6q,2o9s,2opm,2wjw,5m17,7e2t,6etg,1czy,1c82,5ovc,1uj4,4xtw,1kit,1b93,3lx5,5ajc,2q3z,3sji,5el9,4nrm,4u2w,4usw,4yzu,4io7,2j7a,2v88,4omj,1g8m,1w70,4wmo,6i15,3a73,1iup,3juk,6miq,4ndu,3run,6cwm,5mxf,6i44,4kn1,6o0l,2y78,3tf6,6zyj,4tpr,6aco,2ixe,3bf1,3c10,4oti,6w1i,4bdi,6ft7,4xas,5abe,5njx,3p0q,3pkn,3p8o,6zwi,4z2l,1mh5,6g46,1hyv,6mlh,3p1i,1kgw,3hjs,3gpo,6cmj,3qti,4i74,1h2t,3s7k,4uxu,4yyi,5vvg,5n7b,4g37,1evh,6xts,1x06,6dz2,3k2o,3kan,6o5u,3m94,2nl9,6ucn,6zyr,1pdq,6qya,6q8a,2wik,5kgn,2v3u,5v60,4idz,4emx,2jg3,5al1,2wmr,5ur6,5sym,2ylp,4iie,3n8d,1kp8,3tib,5gmh,4qtb,6kjc,6qgg,4jpy,5u94,2o1u,2afw,3cne,5s8q,5h1u,2bmv,3ncg,3rw9,1thz,7k6s,2w9r,6sge,2a8u,5hvp,4kxb,5dms,2wkk,5mk4,6ffe,4ibc,3f39,5pnv,5hcl,4dwb,5d9o,5ah4,2ymt,3fe9,7agd,4l2o,4yih,3pgu,4tlt,5kv8,1xk5,1kwv,2ci9,6pi6,3rew,6mnh,1ax0,5y7x,3q2h,6fh1,5xzf,4ayp,4wno,6u4j,5m7y,2p0c,4uqo,5xva,1wb0,4c1h,1af6,4azt,3fju,5oyd,3hkw,6aao,3pcl,6gy5,1i9s,5xob,6nem,1kbr,2ivz,1d1p,3iqi,6y6j,4mzh,3rps,2j9f,2vl8,6qw1,3q7q,4n5t,4yym,6x8h,6tbk,4p35,1khp,6h75,2p1c,6oko,6znv,3ao4,1ct1,6c0t,5xig,3p7h,4u0w,4j26,6mji,6da1,4lps,1kli,4oks,4rn1,5tpx,4tmt,3qxj,5j28,6clv,4c3l,6hp0,2o88,3f78,5l77,5fnq,4e3b,1nje,5iql,5jmq,5ivq,1l6y,5xp3,7o50,5n55,3ho9,3tif,2yjq,1t7d,5fwj,4sga,4ipz,1ogc,3s68,3o0g,3a1e,5efh,1tcx,2j90,5ifu,3rw8,3m9f,3cke,3sv9,3c0z,4kax,3qi9,2wwp,7etl,2oph,2vtm,4eoy,3mwe,5tc7,2wos,3mlb,2qw1,5x02,2iw4,3o2b,6euz,5fml,6h9x,5ijr,6dlx,4pid,4rse,2x2j,6x7r,6maj,5vyy,5y8z,5zbz,3o64,6g02,5hz9,5y5e,4ff7,6ami,5t8g,4g16,6lzt,3kfn,6ek3,4o9s,4uoh,6j72,4k77,1t46,3jrs,1dhj,5b6c,2bz8,5t2e,6cjj,6ytw,1flm,6ycw,3dri,2vm9,3edh,4oyk,1kdn,1kvo,1g6s,5ngz,6y7k,1u32,4io2,3hkv,2x09,6g84,1ryh,6hy7,6hk6,5o4z,4n7i,3pgl,4c7t,3i8v,4qn7,4hj2,3zj6,6ha4,4fs3,4ynl,4ge2,5mzg,5n2f,6v9k,4w9n,5org,1elr,3gww,1iep,1zp5,3m56,4cgq,6nti,4cup,3rdv,4wci,1ddu,3szi,1h6h,3nw5,3th0,4nzn,6nlj,5ljc,3eks,4odq,1zm7,4czs,4u7k,1rbo,3v31,4ek7,5y9z,3vqz,1x8b,5jjm,6gdy,3bgc,1m7y,1m2x,1a3d,2ltn,5vt1,2uxu,3tay,4k1e,5ok3,2ra6,6faa,2biv,5e8w,6qvg,6syf,1vdf,4fbe,4ijx,4tw9,3qx8,2gs3,6cn8,6pze,4h2z,4ely,5ect,2vzr,3ufa,2z3h,2it4,4jzb,3upy,4lq9,5zg0,1zsb,2wuh,5lt6,1iau,3ap7,6c5h,2pnx,1n51,5ku9,3n45,5y6e,4ps0,3pvu,3pdt,1pum,3d9o,6s07,4q93,5vjd,2fzc,4lrr,3nm6,4mss,4r53,5z5f,1t76,4oeu,1hyo,4omk,3pgp,5ckd,6oin,3qyo,3ti4,3oe1,1qjj,1nw5,3itu,1dgm,3g1v,4u9l,4fl1,3lq2,3kvw,4u4s,4ckj,2f8g,2fkf,1fzq,4muv,3rer,1f2o,4ih3,5ovz,5vza,3psl,6x4j,3tb6,4rd6,3rsr,6zzw,6p10,4do3,5ajz,7kd8,4yml,4y6s,2qwb,3dow,4zsm,2jdy,2vx9,3pfp,4yrr,6bmr,6mli,4oem,6f91,3ta2,1sbr,1d4t,3vi2,5nka,3q5h,4x3k,3dyo,2p1f,1yp6,5ndb,3ivq,1x07,4a5r,5wef,6yjm,3g3r,2dw5,2w8w,3nza,6fty,3vzd,4p5z,2wfi,2toh,4hvc,5fus,4qmx,3hl8,5ne5,4i6b,3cja,2jg2,5u66,5l23,5t26,6c98,5dnj,5lv2,5om2,2wzs,3bbf,4rra,4ur9,1u2y,4qtc,5hwu,5xp6,5dlv,4kcx,6fba,4gbd,2h61,3bhd,1ulg,3hky,6yiz,3gcd,2gvv,2wq5,5dh3,5abw,1me8,5i60,5vbq,4osf,5gv2,5xkm,1eoa,4nhx,5utn,3ud9,5v4q,3g2y,4c1f,4b8y,1ghb,4u0a,1gzc,5vwm,5oai,1khf,5lso,1fwe,4xue,3ivb,2or4,5h14,5lqs,4zhy,3ebb,1k4d,1ekx,3kqa,3qfz,1l8t,3axm,3a1s,3njo,1h60,1a5v,6nc1,3f66,3zqi,6iik,2a3a,5q1g,4bk7,3sm1,4p2t,4jvn,4v11,3qo3,1lii,5drc,3mss,4fxq,4ibm,4jym,6rgr,2ga9,6iyv,4az5,6exj,7xu8,4za0,3f03,3ump,6eks,6os5,6rnt,3ff3,6jfo,2wpb,2nnx,6qri,1ajp,4hhv,6z50,5gof,4gwk,3n0h,4k6w,6l57,3ed0,4oy3,5fog,5j5d,6qlw,4mc2,1gz4,6kdr,6rrv,4y94,2zsc,3g02,6ffs,5ief,6ww1,6dys,3v3q,5eld,2cbz,3gf2,4k1j,5wk9,4gki,3a6v,3mvj,6hgq,6q8k,6mm5,4s1o,1nzv,1nhw,4cd5,4kqr,6f1k,5kva,3t2w,4la7,4pov,2ccb,1i92,5dab,3l0n,6p7q,3pr0,1agw,5ld8,5om9,3o4p,1wcq,4mo5,2why,4x13,1lbk,5kr7,5u0w,2e2q,1kfe,4ymg,5ih6,6y0a,4aua,1t08,1jwy,5aer,4u0y,3i3c,1kax,2om2,3gwx,5v2l,4ccg,3fvy,3hzd,5tdr,3d2f,6vje,5cyv,5yfs,1pkx,4mzf,1iub,3qtc,5acw,5y2s,4rr9,4lng,2j4k,4mpx,5g42,6v4g,1q9d,2w97,2bg1,5j32,5ii2,5sd6,5jr2,6bvb,1kpa,6b7b,2sim,4h88,5aol,4jt9,5fe6,4udy,6n5z,5c3p,4u0e,1gzg,4gv8,3rde,2bv4,4yog,3llp,6dxw,2o1c,2wbg,6jfk,3uwk,6r8p,5nn8,6cz3,3kn4,4qnk,1lmt,4d8s,4tl1,6bq0,6giu,1t1s,6hah,4u43,5dcb,4tq3,4r3v,5std,1ybo,1zkn,2x6x,1i75,6yf2,4rdn,4mk0,1bxr,1a0s,2nmx,1pw1,6e6m,3rl4,3n9j,4au2,3a9i,1moq,6k2n,1atr,6gzl,3blj,4tw6,2bcg,1kc7,6ta2,2one,3t6r,4q9s,3b2t,3n3h,6rtw,5eef,2nnd,4wh7,4wz6,1l3r,6z21,1hy7,4cd1,4u36,4dyk,3alu,5u38,6ap7,5qqc,1fl1,3wci,3ocl,3ofm,3fm5,6dat,3nmn,3trk,2z8e,4htp,4qbt,4qxk,4os5,4eh8,1kee,2j9l,1glg,5v7i,1kre,5wzw,6cbg,6ztc,7s16,1qpb,5yqw,1k1y,4in9,5oxn,3l29,1kxg,4ury,4yad,4wmy,6czd,5xxh,1f4e,5mtw,5xco,6zef,4z2b,5lxi,2qrl,2w87,5im3,5uqs,5ko1,5w2q,6ntb,1rwx,5wlo,2r8q,5azh,2rcn,3f6e,6mxb,2y66,3szb,3pab,5yas,4o1g,5v2q,2j4j,5yco,5yqn,2vk6,5yto,5hm3,1pyd,4kp8,3qpg,5tbj,6mey,3pff,3fpa,1dkd,5z5h,5n1p,2hdq,5tgk,1h4f,3s1y,6r49,4a9c,5hn7,2gqn,5w2h,5a6n,6xxc,4fe9,6c5f,3rlz,4p4t,6hcu,2a5a,6dui,2je8,4aa7,3avs,6n93,4iir,3pz3,1u5r,4pri,4bb4,3b4p,3qi3,6ihv,1cgt,4hzr,4k3k,4by3,3nok,3w8o,6peu,6c86,3i31,4psq,6qau,6n54,4pin,2rc8,4nu0,3rl5,4ag2,3ucn,3zyr,1h65,3otu,6k2o,6zw1,1lds,4ua6,4pkr,1qy2,6r4v,6dyn,3lvv,1nwl,4guj,4b60,3fk1,3n7h,1odl,1fo4,6ipm,1km5,6qmj,3fv3,6uy1,3acw,3ki0,1m0n,4jwk,6gvr,4phn,2wec,1ukt,3muk,2gc8,1gz1,4u03,6bu0,3n9s,4cb5,6dik,6yd7,4bi6,1h10,1qf4,4pyk,4hnn,6qtq,4pfu,3eeb,3ewc,2uw3,5aan,3a09,2yi1,2jgs,5mes,3itc,4uwy,1pfb,2xp3,5z4h,1k1x,6mlg,3qyy,4a2a,5wcm,5w8r,2hah,4led,5l9h,5njw,2i3h,3zi8,6wmd,2hqu,1kic,5lhu,5fp3,4qh8,1m48,5olk,2f1w,5odu,4nmx,2wq4,5y9l,5cuh,4zla,6z6z,7o4p,6yyf,2gfj,4m0e,3ked,7nam,5lzh,4il8,5y7w,5l2n,3q2g,6vgc,4ii9,4uof,5cls,5tvj,1u59,1jif,5mhp,1djx,6blx,4zzy,5yfj,5dv4,2hrm,4xwx,3qkd,5zxk,6ary,4u6e,1f9g,5mxm,6ovz,3w5t,3ucj,7kng,3q30,3m5o,1f73,4nb4,3ngq,4w50,4uy1,2odb,3pd1,3b2q,6h9v,1r17,3zst,2yog,4fxp,1o6i,4h8r,4le7,6rqk,3umq,3adv,1cel,3gg3,2yfa,5hzx,3afj,4ny3,4mp2,7cm8,1lom,4hzv,2o3z,3oui,4uu6,4u46,4w97,1ynu,1ii6,1sv3,4j2v,2c3f,5xs8,6ial,4qel,1o4m,5ixe,4cu1,3kx1,4r8q,5ele,4jck,4j8t,2cje,4gkh,5gvd,2vpb,4cd4,3zmj,3bmo,6e8k,2f28,3pj2,3m3r,3r42,3obq,1apv,6xq6,5oh9,6p7p,4xu3,4aq6,1ucn,3tku,5om8,2cia,1ir1,4mo4,3ncp,3akm,5t4v,3q4z,1ebg,1fcx,2izr,4ywy,3pqz,2e2p,4m2a,5w8v,5wci,5b5q,3rqd,4azc,5iz6,1iag,2qpu,6tnc,4ufx,1qsc,1i7g,2fom,2pxr,6g28,2pgl,1ag9,1pdz,4afy,5nai,5xmq,3hhd,3qla,2z97,7z8w,5afw,5wbq,4mzg,5c5h,1r0x,1hfc,1q1g,6twx,2qin
